A Theoretical Framework for AI Models Explainability with Application in Biomedicine

EXplainable Artificial Intelligence (XAI) is a vibrant research topic in the artificial intelligence community, with growing interest across methods and domains. Much has been written about the subject, yet XAI still lacks shared terminology and a framework capable of providing structural soundness to explanations. In our work, we address these issues by proposing a novel definition of explanation that is a synthesis of what can be found in the literature. We recognize that explanations are not atomic but the combination of evidence stemming from the model and its input-output mapping, and the human interpretation of this evidence. Furthermore, we fit explanations into the properties of faithfulness (i.e., the explanation being a true description of the model's inner workings and decision-making process) and plausibility (i.e., how much the explanation looks convincing to the user). Using our proposed theoretical framework simplifies how these properties are operationalized and it provides new insight into common explanation methods that we analyze as case studies.

==> 08_future_work.tex <==
\section{Future Work}
\label{sec:future-work}

The novel framework proposed in this work makes it clear that the \ac{XAI} community must still face many challenges before claiming the explainability of a model. 
First, we observe an abundance of evidence for explaining black-box models.
Yet, generating faithful interpretations is hard, as much as it is simple to be deceived by plausible yet untrue interpretations.
Secondly, even if an interpretation might be correct (\textit{i.e.}, faithful), it still has to be wrapped in such a way that it is easy for the stakeholders to digest. 
These implications wink at working on explainability from a novel perspective. 
That is, explainability should be part of the software design and engage the stakeholders at the earliest stages of the development of an AI-based tool. 
Future research will need to address the problem of generating faithful interpretations, possibly envisioned through a top-down model design that accounts for explainability as much as it accounts for accuracy. 
Moreover, user studies should be integrated into the explainability design to understand how to deliver explanations that are faithful, possibly plausible, and certainly human-understandable. 
Going a step further, multiple explanation designs should be tested for their effectiveness in enabling the users to perform their tasks in an informed manner, which is the ultimate goal of explainability. 

